UrbanFM: Inferring Fine-Grained Urban Flows

Urban flow monitoring systems play important roles in smart city efforts around the world. However, the ubiquitous deployment of monitoring devices, such as CCTVs, induces a long-lasting and enormous cost for maintenance and operation. This suggests the need for a technology that can reduce the number of deployed devices, while preventing the degeneration of data accuracy and granularity. In this paper, we aim to infer the real-time and fine-grained crowd flows throughout a city based on coarse-grained observations. This task is challenging due to two reasons: the spatial correlations between coarse- and fine-grained urban flows, and the complexities of external impacts. To tackle these issues, we develop a method entitled UrbanFM based on deep neural networks. Our model consists of two major parts: 1) an inference network to generate fine-grained flow distributions from coarse-grained inputs by using a feature extraction module and a novel distributional upsampling module; 2) a general fusion subnet to further boost the performance by considering the influences of different external factors. Extensive experiments on two real-world datasets, namely TaxiBJ and HappyValley, validate the effectiveness and efficiency of our method compared to seven baselines, demonstrating the state-of-the-art performance of our approach on the fine-grained urban flow inference problem.

==> table/minipage.tex <==
\begin{figure}
\begin{minipage}[b]{0.22\textwidth}
  \centering
  \includegraphics[width=\textwidth]{img/fig_percentage.png}
  \caption{figure}
  \vspace{-0.8em}
\end{minipage}
%\hfill
\begin{minipage}[b]{0.22\textwidth}
  \centering
  \small
  \tabcolsep=1mm
  \begin{tabular}{lcccc}\hline
    Method & 10 & 30 & 50 & 100\\ \hline
    SRResNet & 20 & 20 & 20 & 20  \\
    SRResNet-CL & 20 & 20 & 20 & 20\\
    UrbanFM & 20 & 20 & 20 & 20\\
    UrbanFM-NE  &20 & 20 & 20 &20\\\hline
    \end{tabular}
    \vspace{5mm}
    \caption{table}
  \end{minipage}
\end{figure}
%\end{minipage}
